Learning Compact Representations of Neural Networks using DiscriminAtive Masking (DAM)

A central goal in deep learning is to learn compact representations of features at every layer of a neural network, which is useful for both unsupervised representation learning and structured network pruning. While there is a growing body of work in structured pruning, current state-of-the-art methods suffer from two key limitations: (i) instability during training, and (ii) need for an additional step of fine-tuning, which is resource-intensive. At the core of these limitations is the lack of a systematic approach that jointly prunes and refines weights during training in a single stage, and does not require any fine-tuning upon convergence to achieve state-of-the-art performance. We present a novel single-stage structured pruning method termed DiscriminAtive Masking (DAM). The key intuition behind DAM is to discriminatively prefer some of the neurons to be refined during the training process, while gradually masking out other neurons. We show that our proposed DAM approach has remarkably good performance over various applications, including dimensionality reduction, recommendation system, graph representation learning, and structured pruning for image classification. We also theoretically show that the learning objective of DAM is directly related to minimizing the L0 norm of the masking layer.

==> figures/background.tex <==

\section{Backgrounds and Related Works}
\textbf{Unstructured Pruning:}\ 
Pruning individual parameters.
\begin{itemize}
    \item Lottery Ticket Hypothesis
    \item Sparsity-inducing Regularization Schemes
\end{itemize}
\textbf{Structured Pruning:}\ 
Predefined structured pruning
\begin{itemize}
    \item L1-norm based Filter Pruning
\end{itemize}
Automatic structured pruning (Automatic in DAM)
\begin{itemize}
    \item Network sliming
    \item Sparse Structure Selection
\end{itemize}

\begin{equation}
\begin{bmatrix}
 \bm{x_1}&  g_1(\bm{x_1})&  g_2(\bm{x_1})& g_3(\bm{x_1})\\ 
 \bm{x_2}&  g_1(\bm{x_2})&  g_2(\bm{x_2})& g_3(\bm{x_2})\\ 
 ...&  ...&  ...& ...\\ 
 \bm{x_n}&  g_1(\bm{x_n})&  g_2(\bm{x_n})& g_3(\bm{x_n})
\end{bmatrix}
\end{equation}


